Generalization Bounds for Magnitude-Based Pruning via Sparse Matrix Sketching

In this paper, we derive a novel bound on the generalization error of Magnitude-Based pruning of overparameterized neural networks. Our work builds on the bounds in Arora et al. [2018] where the error depends on one, the approximation induced by pruning, and two, the number of parameters in the pruned model, and improves upon standard norm-based generalization bounds. The pruned estimates obtained using our new Magnitude-Based compression algorithm are close to the unpruned functions with high probability, which improves the first criteria. Using Sparse Matrix Sketching, the space of the pruned matrices can be efficiently represented in the space of dense matrices of much smaller dimensions, thereby lowering the second criterion. This leads to stronger generalization bound than many state-of-the-art methods, thereby breaking new ground in the algorithm development for pruning and bounding generalization error of overparameterized models. Beyond this, we extend our results to obtain generalization bound for Iterative Pruning [Frankle and Carbin, 2018]. We empirically verify the success of this new method on ReLU-activated Feed Forward Networks on the MNIST and CIFAR10 datasets.

==> dfi.tex <==
\section{Distance from Initialization}
In order to limit the number of possible parameteriziations of $\hat{M}$ we have to union bound over, we may try to realize that $\mathbf{A}^l \in \mathcal{P}^l$ where $\mathcal{P}^l \subset \mathbb{R}^{d_1^l \times d_2^l}$ is a much smaller subset. One idea from \cite{Neyshabur2018} is to assume that any unit $\mathbf{A}_{i,j}^l$ moves from its starting point $\mathbf{N}_{ij}^l$ on the order of $\frac{1}{d_1^l}$.

\begin{assumption}
\label{ass:ntk}
    We will assume that any element $\mathbf{A}_{ij}^l$ moves within a radius of $\|\mathbf{A}_{ij}^l - \mathbf{N}_{ij}^l\|_2 \leq \frac{1}{d_1^l}$ where $\mathbf{N}_{ij}^l$ is the initialization. 
\end{assumption}
Given a set distance from initialization, we can use \cite{Bartlett2017} to demonstrate a smaller covering number for the number of possible $M$ that can be generated from our learning algorithm.
\begin{theorem}
\label{thm:frombartlett}
    \textbf{Theorem 3.3 from \cite{Bartlett2017}} Let fixed nonlinearities $(\sigma_1, \cots, \sigma_L)$ and initialization matrices $(M_1, \dots, M_L)$, where $\sigma_i$ is $\rho_i$-Lipschitz and $\sigma_i(0) = 0$. Let spectral norm bounds $(s_1, \dots, s_L)$, and matrix $(2,1)$ norm bounds be given. Let $\mathcal{H}_X$ denote the faily of matrices obtained by evaliuating $X$ with all choices of our model $M$:

    $$\mathcal{H}_X \coloneqq \left \{ \mathbf{M}(X^T): \mathcal{A} = (\mathbf{A}_1, \dots, \mathbf{A}_L), \norm{\mathbf{A}^l}_{\sigma} \leq s_l, \norm{\mathbf{A}^l^{\top} - \mathbf{N}^l^{\top}}_{2,1} \leq \frac{1}{d_1^l}\right\}\text{,}$$
    where each matrix has dimension at most $W$ along each axis. Then for any $\epsilon > 0$,
    $$\ln \mathcal{N}(\mathcal{H}_X, \epsilon, \|\cdot\|_2) \leq \frac{\|X\|_2^2\ln(2W^2)}{\epsilon^2} \left(\prod_{j=1}^L s_j^2\rho_j^2\right)\left(\sum_{l=1}^L\left(\frac{1}{d_1^ls_l}\right)^{\frac{2}{3}}\right)^3\text{.}$$
\end{theorem}

Using this bound, we get that 
Therefore, using such a bound, we can bound the generalization of our model as 
\begin{restatable}{theorem}{badgeneralization}
    \label{thm:badgeneralization}
    The generalization of our model is $$L_0(g_A) \leq \hat{L}_{\gamma}(f) + \sqrt{\frac{\ln\left(\sqrt{\frac{J}{\delta}}\right)}{m}}$$
    where $J = \prod_{l=1}^L {d_1^ld_2^l \choose \alpha } \operatorname{exp}\left(\frac{\|X\|_2^2\ln(2W^2)}{\epsilon^2} \left(\prod_{j=1}^L s_j^2\rho_j^2\right)\left(\sum_{l=1}^L\left(\frac{1}{d_1^ls_l}\right)^{\frac{2}{3}}\right)^3\right)$.
    Here $\alpha$ is a probabilitsic upper bound on the number of parameters.
\end{restatable}
This is notably a very bad generalization bound. In fact, using sparsity here makes our generalization bound worse. We can do better. 
